Tensor Fusion Network for Multimodal Sentiment Analysis

Multimodal sentiment analysis is an increasingly popular research area, which extends the conventional language-based definition of sentiment analysis to a multimodal setup where other relevant modalities accompany language. In this paper, we pose the problem of multimodal sentiment analysis as modeling intra-modality and inter-modality dynamics. We introduce a novel model, termed Tensor Fusion Network, which learns both such dynamics end-to-end. The proposed approach is tailored for the volatile nature of spoken language in online videos as well as accompanying gestures and voice. In the experiments, our model outperforms state-of-the-art approaches for both multimodal and unimodal sentiment analysis.

==> fig/Introfig.tex <==
%------------------Overview FIGURE--------------

\begin{figure*}[t!]
	\centering
    \resizebox{16cm}{!}{\includegraphics{fig/model.pdf}} %\input{fig/model.tex}
    \caption{Overview of proposed MCNF Model}
    \label{fig:model}
\end{figure*}


%-----------------------------------------------



==> fig/MOSIfig.tex <==
%------------------MOSI FIGURE------------------
\begin{figure*}[ht!]
	\centering
	\includegraphics[scale=0.4]{MOSIfig1.pdf}
    \caption{Examples from the MOSI dataset.}
    \label{fig:dataset}
\end{figure*}
%-----------------------------------------------

==> fig/va.tex <==
%------------------Motivation FIGURE--------------

\begin{figure}[t]
	\centering
{\includegraphics[width=\linewidth]{fig/va_model.pdf}} 
    \caption{Visual Embedding Subnetwork ($\mathcal{U}_l$)}
    \label{fig:motivation}
\end{figure}


%-----------------------------------------------





==> tables/FeatureDescription.tex <==
\begin{table*}[t!]
  \begin{center}
  \begin{tabular}{  m {3.5cm} | m {11.5cm} } 
  Feature & Description \\ \hline \hline
  Basic Emotions & Set of six basic emotions including anger, contempt, disgust, fear, joy, sadness, and surprise \cite{ekman1992argument}.  \\ \hline
  Advanced Emotions& The two emotions of frustration and confusion better citation \cite{ekman1992argument} \\ \hline
  Facial Action Units& Movements of individual facial muscles are encoded by Facial Action Units which are tightly connected to emotions \cite{ekman1980facial}.  \\ \hline
  Head Pose& The 3D position and rotation parameters of the head, closely related to gaze and gaze aversion \cite{baltruvsaitis2016openface}.  \\ \hline
  Facial Landmarks& Set of 68 important facial feature and outline points \cite{baltruvsaitis2016openface, zadehdclm}   \\ \hline
  yolo& yolo  \\ \hline
  yolo& yolo  \\ \hline



   \end{tabular}
  \captionof{table}{Description of various visual and audio features used in the present work. }
  \label{table:features}
  \end{center}
\end{table*}


==> tables/ResultsTable.tex <==
\newcolumntype{C}[1]{>{\centering\small}m{#1}}
\newcolumntype{?}{!{\vrule width 1.5pt}}
\begin{table*}[t!]
  \begin{center}
  \begin{tabular}{ c ? >{\small}m{5.2cm} ? C{1.4cm} | C{1.4cm} ? C{1.4cm} ? C{1.4cm} | C{1.4cm}  }
  	\cline{3-7}
  	& &\multicolumn{2}{c?}{Binary} & {\normalsize 5-class} &\multicolumn{2}{c|}{Regression}  \tabularnewline\cline{3-7}
    
	& \centering{\normalsize Method} &Accuracy  & F-score  &
    Accuracy & {$\textrm{MAE}$}    & \multicolumn{1}{c|}{\small $r$} \tabularnewline \hline \hline
    
	 
     &Random & 50.2&48.7 & 23.9& 1.367 & -\tabularnewline \Xhline{1.5pt}
     
    \multirow{ 7}{*}{\rotatebox[origin=c]{90}{Language}} &SVM-language \cite{zadeh2016multimodal}&73.1&75.0 &35.1& 1.033 &0.582\tabularnewline  \cline{2-7}
    &RNTN \cite{socher2013recursive} & 73.7&73.4&35.2& 0.987   & 0.592\tabularnewline \cline{2-7}
    &DAN \cite{iyyer2015deep} & 73.4 (68.8)&73.8 (68.4)&39.2 (36.7)&- & -  \tabularnewline \cline{2-7}
    &DynamicCNN \cite{kalchbrenner2014convolutional}& 65.5 (62.1)&66.9 (56.4)&32.0 (32.4)&- & -  \tabularnewline \cline{2-7}
    %&TREE-LSTM CITE & - & -&-&-&-  \tabularnewline \cline{2-7}
    &SAL-CNN-language  \cite{wang2016select} & 73.2 &-&-&-&-  \tabularnewline \cline{2-7}
    &MCNF-language&74.8&75.6 &38.5& 0.989 &0.614\tabularnewline \Xhline{1.5pt}
    
    
    \multirow{ 3}{*}{\rotatebox[origin=c]{90}{Acoustic}}&SVM-audio \cite{zadeh2016multimodal}&63.0&65.5  &25.5& 1.250 & 0.345\tabularnewline \cline{2-7}
	&SAL-CNN-audio \cite{wang2016select} & 61.8&-&-& - &-  \tabularnewline \cline{2-7}
	&MCNF-audio& 65.1&67.3  &27.5& 1.239 & 0.367\tabularnewline \Xhline{1.5pt}
    
    
    \multirow{ 3}{*}{\rotatebox[origin=c]{90}{Visual}}&SAL-CNN-video \cite{wang2016select}&63.6&-&-&-&-  \tabularnewline \cline{2-7}
    &SVM-video \cite{zadeh2016multimodal}&69.4&71.4 &31.0& 1.120 &0.504 \tabularnewline \cline{2-7}
    &MCNF-video& 66.8&70.4  & 30.4 & 1.138 & 0.484\tabularnewline \Xhline{1.5pt}


    \multirow{8}{*}{\rotatebox[origin=c]{90}{Multimodal}}&SAL-CNN \cite{wang2016select} & 73.0 &-&-&-&-  \tabularnewline \cline{2-7}
    &MCNF-SVM &74.0&75.2 &35.2& 0.964 & 0.632 \tabularnewline \cline{2-7}
    &MCNF-early &75.2&76.2 &39.0& 0.942 & 0.648 \tabularnewline \cline{2-7}
    &MCNF-early-35k &75.6&76.8 &38.5& 0.961 & 0.636 \tabularnewline \cline{2-7}
    &MCNF-early-70k &75.2&76.7 &37.6& 0.986 & 0.615 \tabularnewline \cline{2-7}
    &MCNF-early-extra & 75.5 & 76.8&38.8&0.955&0.641 \tabularnewline \cline{2-7}
    &MCNF-(bi)modal &75.3&76.2 &39.7& 0.928 & 0.658 \tabularnewline \cline{2-7}
    &MCNF-(bi+uni)modal &75.2&76.0 &39.6& 0.919 & 0.661 \tabularnewline \cline{2-7}
    &MCNF-(tri)modal & 74.5&75.0&38.9& 0.934 & 0.656\tabularnewline \cline{2-7}
    &MCNF-full &\textbf{76.6}&\textbf{77.6} &\textbf{40.4}& \textbf{0.909} & \textbf{0.674} \tabularnewline \Xhline{1.5pt}
    &Human &85.7&87.5 &53.9& 0.692 & 0.830\tabularnewline \hline
    
  \end{tabular}
  \captionof{table}{Comparative performance of the models evaluated during our experiments. The MCNF-full method (Figure \ref{fig:model}) shows the best performance among our unimodal and multimodal approaches. MAE (Mean Absolute Error, lower is better) and $r$ (Pearson's Correlation) are evaluation metrics for regression (sentiment values $\in [-3,3]$). Fine-grained sentiment analysis is performed over five sentiment classes (section \ref{sec:dataset}) and evaluated using accuracy. Binary classification is evaluated using accuracy and F-score.}
  \label{table:results}
  \end{center}
\end{table*}

==> tables/ex2_table.tex <==
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\begin{comment}


\begin{table}
\small
\setlength\tabcolsep{0.5pt}
\begin{center}
\begin{tabular}{ L{2cm} C{1.1cm} C{1.1cm} C{1.1cm} C{1.08cm} C{1.08cm}}
	\toprule
    %\multicolumn{1}{c}{} & \multicolumn{2}{|c|}{Binary} & \multicolumn{1}{c}{5-class} & \multicolumn{2}{|c|}{Regression} \\
	%\hline
	%Baseline&Acc & F1 & Acc & MAE & $r$ \\ 
    
\multirow{ 2}{*}{Baseline} & \multicolumn{2}{c}{Binary} & \multicolumn{1}{c}{5-class} & \multicolumn{2}{c}{Regression} \\
    \cmidrule(lr{.5em}){2-3} \cmidrule(lr{.5em}){4-4} \cmidrule(lr{.5em}){5-6}
	&Acc(\%) & F1 & Acc(\%) & MAE & $r$ \\
    \midrule

  	\mns & $\mathbf{77.1}$ & $\mathbf{77.9}$ & $\mathbf{42.0}$ & $\mathbf{0.87}$ & $\mathbf{0.70}$\\
  	\midrule
    $\Delta_{E2}$ & $ \uparrow 1.9$ & $\uparrow 1.7$ & $\uparrow 3.0$ & $ \downarrow .09$ & $\uparrow  .07$\\
    \bottomrule
\end{tabular}
\end{center}
\caption{Experiment 2 -- comparison of \mns \ with it's variants that use concatenation fusion instead of Tensor Fusion. \mns \ proves to be a better fusion strategy for combining language, visual and acoustic modalities.} \label{table:earlyres}
\end{table}

\end{comment}



==> tables/mosi_table.tex <==
% \usepackage{multirow}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\begin{table}[]
\centering
\begin{tabular}{|@{}p{5.9cm}|@{}c@{}|}
\hline
Total number of opinion segments &\ 2199\ \\ \hline
Total number of videos & 93 \\ \hline
Total number of distinct speakers  & 89  \\ \hline
Average number of opinion segments in video & 23.2 \\ \hline
Average length of opinion segments (sec.) & 4.2 \\ \hline
Average word count per opinion segments & 12  \\ \hline
Total number of words in opinion segments & 26295 \\ \hline
Total of unique words in opinion segments & 3107 \\ \hline
Total number of words in opinion segments appearing at least 10 times in the dataset & 557 \\ \hline
\end{tabular}
\caption{CMU-MOSI dataset statistics.}\label{table:mosistat}
\end{table}
